Style Transfer as Data Augmentation: A Case Study on Named Entity Recognition

In this work, we take the named entity recognition task in the English language as a case study and explore style transfer as a data augmentation method to increase the size and diversity of training data in low-resource scenarios. We propose a new method to effectively transform the text from a high-resource domain to a low-resource domain by changing its style-related attributes to generate synthetic data for training. Moreover, we design a constrained decoding algorithm along with a set of key ingredients for data selection to guarantee the generation of valid and coherent data. Experiments and analysis on five different domain pairs under different data regimes demonstrate that our approach can significantly improve results compared to current state-of-the-art data augmentation methods. Our approach is a practical solution to data scarcity, and we expect it to be applicable to other NLP tasks.

==> figures/data_reliability.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\linewidth]{images/data_reliability.png}
\caption{Performance comparison of different data augmentation methods with infinite amount of pseudo data for training in \textsc{full-set} setting. Scores are calculated with the micro F1 metric.}
\label{fig: data_reliability}
\end{figure*}

==> figures/data_selection.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{images/data_selection.png}
\caption{
Prefix tree based constraints decoding algorithm for sentence generation. 
\texttt{<BOS>} and \texttt{<EOS>} represent the start and the end of each sentence. 
\texttt{<Text>} refers to the text spans while \texttt{<B\_ENT>} and \texttt{<I\_ENT>} refer to the start and inside of entity spans respectively. 
}
\label{fig: data_selection}
\end{figure*}

==> figures/style_transfer_example.tex <==
\begin{figure}[t]
\centering
\subfigure{
    \begin{minipage}[t]{0.97\linewidth}
    \centering
    \includegraphics[width=0.97\linewidth]{example-image-a}
    \end{minipage}
}
\caption{Examples for style transfer as data augmentation. }
\label{fig: style_transfer_example}
\end{figure}

==> tables/error_analysis.tex <==
\begin{table*}[t!]
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{@{}llll@{}}
\toprule
\textbf{\#} 
    & \textbf{Original Sentences (formal)} 
    & \textbf{Generated Sentences (informal)} 
\\\toprule

1 & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    The departing Mr. \textbf{{[}Cathcart{]}\sub{PERSON}} says he has no worries about \textbf{{[}Kidder{]}\sub{ORGANIZATION}} 's future.
\end{tabular} & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    He says he has no worries
\end{tabular}
\\\midrule

2 & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    I don't think the checks are worth \$ \textbf{{[}15{]}\sub{MONEY}} apiece, '' he says.
\end{tabular} &
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    he says It's weird they're for \$ 15 per check 
\end{tabular} 
\\\midrule

3 & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    Well the rescue vehicle if it's required will have only \textbf{{[}four{]}\sub{CARDINAL}} people on it.
\end{tabular} & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    well if necessary the rescue car.. WILL have only four + people on it
\end{tabular}
\\\midrule

4 & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    it's going to be in small gathering places in middle \textbf{{[}America{]}\sub{GPE}} with people saying some pretty horrible things
\end{tabular} & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    Small gathering places in the middle \textbf{{[}America{]}\sub{LOC}} with people saying some pretty awful things
\end{tabular}
\\\midrule

5 & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    So \textbf{{[}al Jazeera TV{]}\sub{ORGANIZATION}} station has also adopted this structure.
\end{tabular} & 
\begin{tabular}[t]{@{}p{0.55\linewidth}@{}}
    Because \textbf{{[}al Jazeera{]}\sub{PERSON}} TV \textbf{{[}Imad{]}\sub{PERSON}} has too follow that structure
\end{tabular} 
\\\bottomrule
\end{tabular}
}
\caption{
Examples of data augmentation with data transformation for error analysis. The sentences are tagged with their corresponding entities in brackets (e.g., {[}Cathcart{]}\sub{PERSON}).
}
\label{tab: error_analysis}
\end{table*}

